ActUp: Analyzing and Consolidating tSNE and UMAP

tSNE and UMAP are popular dimensionality reduction algorithms due to their speed and interpretable low-dimensional embeddings. Despite their popularity, however, little work has been done to study their full span of differences. We theoretically and experimentally evaluate the space of parameters in both tSNE and UMAP and observe that a single one -- the normalization -- is responsible for switching between them. This, in turn, implies that a majority of the algorithmic differences can be toggled without affecting the embeddings. We discuss the implications this has on several theoretic claims behind UMAP, as well as how to reconcile them with existing tSNE interpretations. Based on our analysis, we provide a method (\ourmethod) that combines previously incompatible techniques from tSNE and UMAP and can replicate the results of either algorithm. This allows our method to incorporate further improvements, such as an acceleration that obtains either method's outputs faster than UMAP. We release improved versions of tSNE, UMAP, and \ourmethod that are fully plug-and-play with the traditional libraries at https://github.com/Andrew-Draganov/GiDR-DUN

==> Figures/irrelevant_coil.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    default & frobenius & initialization & a, b scalars & symmetrization & sym attraction & pseudo-distance\\

    \hline

    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/default_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/frob_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/random_init_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/tsne_scalars_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/tsne_symmetrization_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/sym_attraction_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/tsne/umap_metric_embedding.png}\\

    \hline

    \includegraphics[width=.123\linewidth]{outputs/coil/umap/default_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/frob_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/random_init_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/tsne_scalars_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/tsne_symmetrization_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/sym_attraction_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/umap/umap_metric_embedding.png}\\

    \hline

    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/default_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/frob_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/random_init_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/tsne_scalars_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/tsne_symmetrization_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/sym_attraction_embedding.png}&
    \includegraphics[width=.123\linewidth]{outputs/coil/uniform_umap/umap_metric_embedding.png}\\

    \hline
    \end{tabular}
    \caption{Effect of the algorithm settings from Table \ref{differences_table} on Coil-100 embeddings.}
    \label{irrelevant-fashion-mnist}
\end{table*}

==> Figures/relevant_params_fashion_mnist.tex <==
% \begin{figure} \label{relevant-fashion-mnist}
%     \centering
%     \begin{tabular}{|c|c|c|}
%     \hline
%     default & \centered{normalization and \\ gradient amplification} & sym attraction \\
%     \hline

%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/tsne/default_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/tsne/normalized_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/tsne/sym_attraction_embedding.png}\\
%     \hline

%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/umap/default_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/umap/normalized_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/umap/sym_attraction_embedding.png}\\
%     \hline

%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/uniform_umap/default_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/uniform_umap/normalized_embedding.png}&
%     \includegraphics[width=.25\linewidth]{outputs/fashion_mnist/uniform_umap/sym_attraction_embedding.png}\\

%     \hline
%     \end{tabular}
% \end{figure}

==> Figures/usps_embeddings.tex <==
\begin{figure}[ht]
    \centering
    \begin{tabular}{m{0.3em}cc}
        & Unnormalized & Normalized \\
        \makecell{\rotatebox[origin=c]{90}{GDR}} &
        \raisebox{-0.5\height}{\includegraphics[width=3.75cm]{outputs/usps/GDR}} &
        \raisebox{-0.5\height}{\includegraphics[width=3.75cm]{outputs/usps/GDR_normalized.pdf}}\\
        \makecell{\rotatebox[origin=c]{90}{tSNE/UMAP}} & 
        \raisebox{-0.5\height}{\includegraphics[width=3.75cm]{outputs/usps/umap.pdf}} &
        \raisebox{-0.5\height}{\includegraphics[width=3.75cm]{outputs/usps/tsne}}\\
    \end{tabular}
\caption{Embeddings on the USPS dataset.}
\label{usps_plots}
\end{figure}

==> Tables/irrelevant_params_mnist_metrics.tex <==
\begin{table*}[!htb]
    \centering
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \begin{subtable}[t]{\linewidth}
        \begin{tabularx}{\linewidth}{m{1.5cm}|*{7}{c}|c}
        % \toprule
         \textit{Algorithm} & \textit{Original} & Frobenius & Initialization & Pseudo-distance & Symmetrization & Sym attraction & Scalars & \textit{Algorithm mean} \\
        \midrule
        % \multirow{5}{*}{kNN Accuracy}
        UMAP          & 95.4 & 96.7 & 96.6 & 94.4 & 96.7 & 96.6 & 96.5 & 96.3$\pm$1.0 \\ 
        \ourmethodU   & 96.2 & 96.2 & 96.4 & 96.7 & 96.6 & 96.5 & 95.8 & 96.3$\pm$0.3 \\ 
        tSNE          & 95.1 & 94.7 & 95.2 & 96.0 & 94.9 & 94.8 & 95.1 & 95.1$\pm$0.4\\ 
        \ourmethodN   & 96.1 & 96.3 & 95.6 & 96.1 & 96.1 & 96.3 & 96.1 & 96.1$\pm$0.2 \\ 
        \midrule
        \textit{Parameter mean dev.} & -0.3 & 0.1 & 0.0 & 0.1 & 0.4 & -0.7 &  0.4 & \\
        \end{tabularx}    
    \caption{kNN-accuracy}        
    \end{subtable}
    \begin{subtable}[t]{\textwidth}
        \begin{tabularx}{\linewidth}{m{1.5cm}|*{7}{c}|c}
         \textit{Algorithm} & \textit{Original} & Frobenius & Initialization & Pseudo-distance & Symmetrization & Sym attraction & Scalars & \textit{Algorithm mean} \\
        \midrule
        %\multirow{5}{*}{V-score}
        UMAP          & 82.5 & 87.0 & 84.6 & 82.2 & 82.5 & 83.5 & 82.2 & 83.5$\pm$1.6 \\ 
        \ourmethodU   & 84.0 & 85.4 & 82.1 & 85.2 & 85.1 & 83.3 & 81.2 & 83.8$\pm$1.5 \\ 
        tSNE          & 70.9 & 71.8 & 70.7 & 73.9 & 70.8 & 80.7 & 73.5 & 73.2$\pm$3.3 \\ 
        \ourmethodN   & 67.8 & 71.9 & 61.3 & 63.0 & 68.4 & 72.7 & 68.8 & 67.7$\pm$3.9 \\ 
        \midrule
        \textit{Parameter mean dev.} & -1.4 & 2.2 & -2.4 & -1.0 & 1.3 & -1.0 & 1.4 & \\
        \end{tabularx}
    \caption{V-score}    
    \end{subtable}
    \caption{kNN-accuracy ($k=100$) and V-score on MNIST for each parameter. Algorithm mean shows mean and confidence intervals on all the algorithmic changes. 
     \ourmethod successfully produces tSNE and UMAP embeddings across the settings. Parameter mean deviation shows the average difference between each value and the algorithm mean. A value close to 0 means no impact.}
    \label{irrelevant-metrics}
\end{table*}


% \begin{table*}[!htb]
%     \centering
%     \begin{tabularx}{\linewidth}{m{1.8cm}|m{1.5cm}*{7}{c}|c}
%     % \toprule
%     Metric & Algorithm & Default & Frobenius & Initialization & Pseudo-distance & Symmetrization & Sym attraction & Scalars & Algorithm mean \\
%     \midrule
%     \multirow{5}{*}{kNN Accuracy}
%     & UMAP          & 95.4 & 96.7 & 96.6 & 94.4 & 96.7 & 96.6 & 96.5 & 96.3$\pm$1.0 \\ 
%     & \ourmethodU   & 96.2 & 96.2 & 96.4 & 96.7 & 96.6 & 96.5 & 95.8 & 96.3$\pm$0.3 \\ 
%     & tSNE          & 95.1 & 94.7 & 95.2 & 96.0 & 94.9 & 94.8 & 95.1 & 95.1$\pm$0.4\\ 
%     & \ourmethodN   & 96.1 & 96.3 & 95.6 & 96.1 & 96.1 & 96.3 & 96.1 & 96.1$\pm$0.2 \\ 
%     \cline{2-10}
%     & Parameter mean deviation & -0.3 & 0.1 & 0.0 & 0.1 & 0.4 & -0.7 &  0.4 & \\
%     \midrule
%     \multirow{5}{*}{V-score}
%     & UMAP          & 82.5 & 87.0 & 84.6 & 82.2 & 82.5 & 83.5 & 82.2 & 83.5$\pm$1.6 \\ 
%     & \ourmethodU   & 84.0 & 85.4 & 82.1 & 85.2 & 85.1 & 83.3 & 81.2 & 83.8$\pm$1.5 \\ 
%     & tSNE          & 70.9 & 71.8 & 70.7 & 73.9 & 70.8 & 80.7 & 73.5 & 73.2$\pm$3.3 \\ 
%     & \ourmethodN   & 67.8 & 71.9 & 61.3 & 63.0 & 68.4 & 72.7 & 68.8 & 67.7$\pm$3.9 \\ 
%     \cline{2-10}
%     & Parameter mean deviation & -1.4 & 2.2 & -2.4 & -1.0 & 1.3 & -1.0 & 1.4 & \\
%     \bottomrule
%     \end{tabularx}
%     \caption{kNN-accuracy ($k=100$) and V-score on MNIST for each parameter. Row-means are comparable for the pairs [UMAP $\leftrightarrow$ \ourmethodU] and [tSNE $\leftrightarrow$ \ourmethodN]. 
%      \ourmethod successfully produces tSNE and UMAP embeddings across the hyperparameters. The parameter mean deviation shows the average difference between each value and the algorithm mean. The parameter mean deviations being close to 0 implies that each parameter does not significantly impact any of the algorithms.}
%     \label{irrelevant-metrics}
% \end{table*}




==> Tables/original_speeds.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    tSNE & \makecell{Our tSNE} & UMAP & \makecell{Our UMAP} \\
    \hline
    731.5 $\pm$ 22.3 & 430.3$\pm$42.5 & 71.2 $\pm$ 0.8 & 38.9$\pm$0.5 \\
    \hline
    \end{tabular}
    \caption{Runtimes (in seconds) for the original tSNE and UMAP algorithms vs. our implementations of tSNE and UMAP on the MNIST dataset.}
    \label{original_mnist_speeds}
\end{table}

==> authors.tex <==
%%
%% The "author" command and its associated commands are used to define the authors and their affiliations.
\author{Andrew Draganov}
\affiliation{%
  \institution{Aarhus University}
   \country{}
}
\email{draganovandrew@cs.au.dk}

\author{Tyrus Berry}
\affiliation{\institution{George Mason University}
\country{}
}
\email{tberry@gmu.edu}

\author{Jakob Rødsgaard Jørgensen}
\affiliation{%
  \institution{Aarhus University}
    \country{}
}
\email{jakobrj@cs.au.dk}

\author{Katrine Scheel Nellemann}
\affiliation{%
  \institution{Aarhus University}
    \country{}
}
\email{scheel@cs.au.dk}

\author{Ira Assent}
\affiliation{%
  \institution{Aarhus University}
    \country{}
}
\email{ira@cs.au.dk}

\author{Davide Mottin}
\affiliation{%
  \institution{Aarhus University}
    \country{}
}
\email{davide@cs.au.dk}

\author{Cigdem Aslay}
\affiliation{%
  \institution{Aarhus University}
    \country{}
}
\email{cigdem@cs.au.dk}

